Learning of feature points without additional supervision improves reinforcement learning from images

In many control problems that include vision, optimal controls can be inferred from the location of the objects in the scene. This information can be represented using feature points, which is a list of spatial locations in learned feature maps of an input image. Previous works show that feature points learned using unsupervised pre-training or human supervision can provide good features for control tasks. In this paper, we show that it is possible to learn efficient feature point representations end-to-end, without the need for unsupervised pre-training, decoders, or additional losses. Our proposed architecture consists of a differentiable feature point extractor that feeds the coordinates of the estimated feature points directly to a soft actor-critic agent. The proposed algorithm yields performance competitive to the state-of-the art on DeepMind Control Suite tasks.

==> keypoints_fig.tex <==
\begin{figure*}[t]

\begin{subfigure}{.162\textwidth}
\caption{Ball in Cup}
\centering\vspace{-2mm}
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/ball_in_cup_catch/0_gt.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\caption{Cartpole}\vspace{-2mm}
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/cartpole_swingup/10_gt.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\caption{Cheetah}\vspace{-2mm}
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/cheetah_run/0_gt.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\caption{Finger}\vspace{-2mm}
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/finger_spin/10_gt.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\caption{Reacher}\vspace{-2mm}
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/reacher_easy/0_gt.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\caption{Walker}\vspace{-2mm}
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/walker_walk/70_gt.png}
\end{subfigure}

\vspace{1pt}

\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/ball_in_cup_catch/0_pred.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/cartpole_swingup/10_pred.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/cheetah_run/0_pred.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/finger_spin/10_pred.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/reacher_easy/0_pred.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=110 45 110 45, clip]{corl_analysis/walker_walk/70_pred.png}
\end{subfigure}

\vspace{1pt}

\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/ball_in_cup_catch/0_3.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/cartpole_swingup/10_3.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/cheetah_run/0_0.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/finger_spin/10_7.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/reacher_easy/0_0.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/walker_walk/70_2.png}
\end{subfigure}

\vspace{1pt}

\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/ball_in_cup_catch/0_1.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/cartpole_swingup/10_4.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/cheetah_run/0_6.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/finger_spin/10_3.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/reacher_easy/0_6.png}
\end{subfigure}
\begin{subfigure}{.162\textwidth}
\centering
\includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/walker_walk/70_6.png}
\end{subfigure}

% \vspace{1pt}

% \begin{subfigure}{.162\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/ball_in_cup_catch/0_1.png}
% \end{subfigure}
% \begin{subfigure}{.162\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/cartpole_swingup/10_2.png}
% \end{subfigure}
% \begin{subfigure}{.162\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/cheetah_run/0_2.png}
% \end{subfigure}
% \begin{subfigure}{.162\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/finger_spin/10_2.png}
% \end{subfigure}
% \begin{subfigure}{.162\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/reacher_easy/0_2.png}
% \end{subfigure}
% \begin{subfigure}{.162\textwidth}
% \centering
% \includegraphics[width=1.0\linewidth, trim=125 35 93 55, clip]{corl_analysis/walker_walk/70_2.png}
% \end{subfigure}

\caption{
\emph{Row 1}: Example frames from six considered tasks from the PlaNet benchmark. The black crosses represent the handcrafted keypoints extracted from the simulator.
\emph{Row 2}: Keypoints learned by KeyQ with $K=8$.
\emph{Rows 3 and 4}: Some feature maps $h(\cdot,\cdot,k)$ produced by the convolutional KeyQ encoder along with the probability distributions of the keypoint location \eqref{eq:key1d}. Brighter pixels indicate larger values.
KeyQ can learn to represent parts of an object (row 3), multiple objects (by activating the locations of multiple objects as, for example, in row 4 for Finger and Ball in Cup) or the background (row 4 for Cartpole).
%KeyQ learns to use keypoints to represent particular parts of relevant objects (row 3). We observe that KeyQ also uses keypoints to represent the distance between objects that are relevant for the control task. This is achieved by activating the location of multiple objects in the feature map. For example, the distance between the ball and the cup in Ball in Cup (row 4), the distance between the finger and rotatable body in Finger (row 4), and the distance between the front and back legs of Cheetah (row 4) and Walker (row 4). See Fig.~\ref{fig:keypoint-dynamics} for dynamics of these keypoints that track the relative motion between objects.
%We also observe that keypoints are used to segment and represent the background (e.g. Cartpole, row 4).
}
\label{fig:keypoints}

\end{figure*}
